GOCA: Guided Online Cluster Assignment for Self-Supervised Video Representation Learning

Clustering is a ubiquitous tool in unsupervised learning. Most of the existing self-supervised representation learning methods typically cluster samples based on visually dominant features. While this works well for image-based self-supervision, it often fails for videos, which require understanding motion rather than focusing on background. Using optical flow as complementary information to RGB can alleviate this problem. However, we observe that a naive combination of the two views does not provide meaningful gains. In this paper, we propose a principled way to combine two views. Specifically, we propose a novel clustering strategy where we use the initial cluster assignment of each view as prior to guide the final cluster assignment of the other view. This idea will enforce similar cluster structures for both views, and the formed clusters will be semantically abstract and robust to noisy inputs coming from each individual view. Additionally, we propose a novel regularization strategy to address the feature collapse problem, which is common in cluster-based self-supervised learning methods. Our extensive evaluation shows the effectiveness of our learned representations on downstream tasks, e.g., video retrieval and action recognition. Specifically, we outperform the state of the art by 7% on UCF and 4% on HMDB for video retrieval, and 5% on UCF and 6% on HMDB for video classification

==> acknowledgement.tex <==
\section{Acknowledgemen}    \label{sec:acknowledgement}
This work has been supported by the Snap Inc.

==> tbls/abl_lambda.tex <==

\begin{table}[!ht]
	\centering{
	\resizebox{.30\textwidth}{!}{
	\begin{tabular}{
			>{\raggedright\arraybackslash}p{0.5cm}
			>{\columncolor{Res7}}>{\centering\arraybackslash}p{0.6cm}
			>{\columncolor{Res1}}>{\centering\arraybackslash}p{0.6cm}
			>{\columncolor{Res1}}>{\centering\arraybackslash}p{0.6cm}
			>{\columncolor{Res1}}>{\centering\arraybackslash}p{0.6cm}
 		    >{\columncolor{Res1}}>{\centering\arraybackslash}p{0.6cm}}
	  	%\toprule 	
	  	\multicolumn{2}{c}{} & 
	  	\multicolumn{4}{c}{$ \lambda_{1}$} \\  
	  	\cmidrule{3-6}
	  	\multicolumn{2}{c}{} & 
	  	\multicolumn{1}{c}{\small {0.01}} & 
        \multicolumn{1}{c}{\small {0.02}} & 
        \multicolumn{1}{c}{\small {0.03}} & 
        \multicolumn{1}{c}{\small {0.04}}
        \\
% 	  \midrule
     & 0.01 &  56.4 & 57.6 & 55.1 & 54.1 \\
    $ \lambda_{2}$ & 0.02 &  57.3 & 58.7 & \textbf{60.1} & 58.9 \\
    & 0.03 &  58.1 & \textbf{60.9} & \textbf{60.5} & 57.5 \\
     & 0.04 & 55.8 & 58.5 & \textbf{59.0} & 55.2\\
	\bottomrule
	\end{tabular}
	}
	}
	\caption{The effect of lambda parameters on recall values on the RGB-only evaluation at UCF dataset}
		\label{tbl:lambda}
\end{table}



==> tbls/abl_modal_mergeprior.tex <==
\begin{table}[!ht]
	\centering{
	\resizebox{.42\textwidth}{!}{
	\begin{tabular}{
			>{\raggedright\arraybackslash}p{1.4cm}
			>{\columncolor{Res2}}>{\centering\arraybackslash}p{0.75cm}
			>{\columncolor{Res2}}>{\centering\arraybackslash}p{0.7cm}
			>{\columncolor{Res1}}>{\centering\arraybackslash}p{0.8cm}
			>{\columncolor{Res1}}>{\centering\arraybackslash}p{0.8cm}
			>{\columncolor{Res3}}>{\centering\arraybackslash}p{0.8cm}
			>{\columncolor{Res3}}>{\centering\arraybackslash}p{0.8cm}} 	
	  	\multicolumn{3}{c}{} & 
		\multicolumn{2}{c}{\small {UCF}} &  
		\multicolumn{2}{c}{\small {HMDB}}\\
		\cmidrule{4-7}
		\multicolumn{1}{c}{Method} &
		\multicolumn{1}{c}{Train} &
		\multicolumn{1}{c}{Test}
		&\multicolumn{1}{c}{R@1}& \multicolumn{1}{c}{R@5}
		&\multicolumn{1}{c}{R@1}& \multicolumn{1}{c}{R@5}
		\\
	  \midrule
	 SModal &   R  &  R & 41.3 & 58.9  & 17.9 & 43.2\\
	 SModal &   F  &  F & 62.0 & 75.8 & 28.2 & 53.3 \\
	 VICC~\cite{toering2021selfsupervised} &  R+F  &  R & 62.1  &  77.1   & 25.5 & 49.6 \\
     VICC~\cite{toering2021selfsupervised} &  R+F  &  F & 59.7 &  77.3   & 27.7 & 53.3 \\
	 \textbf{GOCA} &  R+F  &  R & 63.4 &  76.3   & 26.3 & 50.2 \\
    \textbf{GOCA} &  R+F  &  F & 67.9 &  79.5   & 31.8 & 56.3 \\
     \midrule
     SModal+ &   -  & R+F & 63.6 & 76.8  & 28.6 & 54.1\\
     Avg &   R+F  & R+F & 50.8 & 63.0  & 22.8 & 46.3\\
     Sep &   R+F  & R+F & 65.0 &  78.2  & 29.5 & 54.8 \\
      \textbf{GOCA+} &  R+F & R+F & 70.8 &  81.4   & 33.7 & 58.7\\
  
	\bottomrule
	\end{tabular}
	}
	}
	\caption{Comparison of \emph{RGB} (R) and \emph{OF} (F) merging strategies}
		\label{tbl:prior}
\end{table}


==> tbls/abl_protreg.tex <==


\begin{table}[!ht]
	\centering{
	\resizebox{.42\textwidth}{!}{
	\begin{tabular}{
			>{\raggedright\arraybackslash}p{1.2cm}
			>{\raggedright\arraybackslash}p{1cm}
			>{\columncolor{Res2}}>{\centering\arraybackslash}p{0.75cm}
			>{\columncolor{Res2}}>{\centering\arraybackslash}p{0.6cm}
			>{\columncolor{Res1}}>{\centering\arraybackslash}p{0.8cm}
			>{\columncolor{Res1}}>{\centering\arraybackslash}p{0.8cm}
			>{\columncolor{Res3}}>{\centering\arraybackslash}p{0.8cm}
			>{\columncolor{Res3}}>{\centering\arraybackslash}p{0.8cm}}
	  	%\toprule 	
	  	\multicolumn{1}{c}{} & 
	  	\multicolumn{1}{c}{Use} & 
	  	\multicolumn{2}{c}{} & 
		\multicolumn{2}{c}{\small {UCF}} &  
		\multicolumn{2}{c}{\small {HMDB}}\\
		\cmidrule{5-8}
		\multicolumn{1}{c}{Method} &
		\multicolumn{1}{c}{ProtReg} &
		\multicolumn{1}{c}{Train}&
		\multicolumn{1}{c}{Test}
		&\multicolumn{1}{c}{R@1}& \multicolumn{1}{c}{R@5}
		&\multicolumn{1}{c}{R@1}& \multicolumn{1}{c}{R@5}\\
	  \midrule
      SModal&\textbf{No} &     R & R &  40.9 & 57.4 & 17.1 & 42.7\\
       SModal&\textbf{Yes} &     R & R & 42.3 & 58.9  & 17.9 & 43.2 \\
      \midrule
	\textbf{GOCA+}& \textbf{No} &     R+F & R+F &  69.1 & 79.4 & 32.9 & 58.6 \\
       \textbf{GOCA+}&\textbf{Yes} &    R+F & R+F &  70.8 &  81.4 & 33.6 & 58.7  \\
	
	\bottomrule
	\end{tabular}}}
	\caption{
	Effect of prototype regularization on recall values}
		\label{tbl:protreg}
\end{table}



==> tbls/fig_prototypes.tex <==

\begin{figure}[!ht]
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[scale=0.1]{files/figures/TrainedProts.png}
  \caption{Trained Prototypes}
  \label{fig:prototypes_sub2}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[scale=0.1]{files/figures/RegProts.png}
  \caption{Regularized Prototypes}
  \label{fig:prototypes_sub1}
\end{subfigure}%
\caption{t-SNE plot of 1000 prototypes in 2D. Figure (a) show random initialization of prototypes. Figure (b) show prototypes that trained with backbone network without any regularizer. These prototypes are randomly initialized as in Figure (a). Figure (c) shows our regularized prototypes.  }\label{fig:prototypes}
\end{figure}


==> tbls/ft.tex <==

\begin{table}[!ht]
	% %\setlength\tabcolsep{2 pt}
	\addtolength{\tabcolsep}{-1.7pt}    
	\centering{
		\resizebox{.40\textwidth}{!}{
	\begin{tabular}{
			>{\raggedright\arraybackslash}p{2.1cm}
			>{\columncolor{Res2}}>{\centering\arraybackslash}p{0.7cm}
			>{\columncolor{Res2}}>{\centering\arraybackslash}p{1.7cm}
			>{\columncolor{Res2}}>{\centering\arraybackslash}p{0.5cm}
			>{\columncolor{Res1}}>{\centering\arraybackslash}p{0.7cm}
			>{\columncolor{Res3}}>{\centering\arraybackslash}p{1.1cm}}
	  
		\multicolumn{1}{c}{Method}
		&\multicolumn{1}{c}{DS} 
		&\multicolumn{1}{c}{Backbone} 
		&\multicolumn{1}{c}{Sz} 
		&\multicolumn{1}{c}{UCF}
		&\multicolumn{1}{c}{HMDB} \\
       
	  \midrule
	   %XDC*~\cite{alwassel_2020_xdc} & K400 & R(2+1)D+18 & 224    & 84.2 &47.1\\
	   %AVSF*~\cite{xiao2020audiovisual} & K400 & SF-50 & 224    & 87.0 & 54.6\\
	   CVRL~\cite{qian2021spatiotemporal} & K400 & R3D-50 & 224   & 92.9 & 67.9\\
	   %MoCo~\cite{feichtenhofer2021large} & K400 &R-50 & 224    & 93.3 & - \\
	   $\rho$ BYOL~\cite{feichtenhofer2021large} & K400 &R-50 & 224     & 95.5 & 73.6 \\
% 	   TaCo~\cite{bai2020can} & K400 & R50 & 224    & 85.1 & 51.6\\
	  \hdashline[5pt/5pt]
	   ASCNet\cite{qian2021enhancing} & K400 & R3D-18 & 112    & 80.5 &  52.3\\
	   Enhanced\cite{qian2021enhancing} & K400 & R3D-18 & 112    & 79.1 &  47.6\\
	   CoCLR~\cite{Han20} & K400 & S3D & 128    & 87.9 & 54.6\\
	   CoCLR+~\cite{Han20} & K400& S3D & 128  & 90.6 &
	   62.9\\
	   
	   
	   \textbf{GOCA} & K400 & S3D & 128    & 89.3 & 63.2\\
	   \textbf{GOCA+} & K400 & S3D & 128    & \textbf{91.1} &
	   \textbf{65.8}\\
	   \midrule
	   \midrule
	   VCOP~\cite{xu2019self} & UCF & R(2+1)D+18 & 112    &  72.4 &  30.9\\
	    
	   %Var. PSP~\cite{cho2021self} & UCF & R3D+18 & 112    &  74.8 &  36.8\\
	      
	   Pace Pred~\cite{wang2020self} & UCF & R(2+1)D+18 & 112     &  75.9 & 35.9\\
	   VCP~\cite{luo2020video} & UCF & R(2+1)D+18 & 112    &  66.3 & 32.2\\
	   PRP~\cite{Yao_2020_CVPR} & UCF & R(2+1)D+18 & 112    & 72.1 & 35.0\\
	   RTT~\cite{jenni2020video} & UCF & R(2+1)D+18 & 112    & 81.6 & 46.4\\
	   Enhanced~\cite{qian2021enhancing} & UCF & R3D+18 & 112    & 76.2 &  41.1\\
	   
	   \textbf{GOCA} & UCF & R(2+1)D+18 & 112     &  82.1 &   54.7\\
	   \textbf{GOCA+} & UCF & R(2+1)D+18 & 112    & \textbf{88.7} &  \textbf{60.1} \\
	 
	  \midrule
	 
	   CoCLR~\cite{Han20} & UCF & S3D & 128   & 81.4 & 52.1\\
	   CoCLR+~\cite{Han20} & UCF & S3D & 128    & 87.3 &  58.7\\
	   ViCC~\cite{toering2021selfsupervised} & UCF & S3D & 128    &  84.3 &   47.9\\
	   ViCC+~\cite{toering2021selfsupervised} & UCF & S3D & 128    & \textbf{90.5} &   62.2\\
	   
	   \textbf{GOCA} & UCF & S3D & 128     &  83.4 &   53.5\\
	   \textbf{GOCA+} & UCF & S3D & 128  & 90.2 &  \textbf{64.8}\\
	   
	\bottomrule
	\end{tabular}}}
	% %\setlength{\abovecaptionskip}{\RemoveAboveCaption}
	\vspace{-3mm}
	\caption{
\emph{Fine Tuning} experimental setup results on on UCF101~\cite{ucf101} and HMDB\cite{hmdb}. 
}
		\label{tbl:ft}
	\vspace{-5mm}
\end{table}


==> tbls/lc.tex <==

\begin{table}[!ht]
    \addtolength{\tabcolsep}{-1.5pt}    
	% %\setlength\tabcolsep{2 pt}
	\centering{
		\resizebox{.36\textwidth}{!}{
	\begin{tabular}{
			>{\raggedright\arraybackslash}p{2cm}
			>{\columncolor{Res2}}>{\centering\arraybackslash}p{0.7cm}
			>{\columncolor{Res2}}>{\centering\arraybackslash}p{1.7cm}
			>{\columncolor{Res2}}>{\centering\arraybackslash}p{0.4cm}
			>{\columncolor{Res1}}>{\centering\arraybackslash}p{0.7cm}
			>{\columncolor{Res3}}>{\centering\arraybackslash}p{1.1cm}}
	    
	   % \multicolumn{6}{c}{Linear Classification} \\
	    
	   % \midrule
		\multicolumn{1}{c}{Method}
		&\multicolumn{1}{c}{DS} 
		&\multicolumn{1}{c}{Backbone} 
		&\multicolumn{1}{c}{Sz} 
		&\multicolumn{1}{c}{UCF}
		&\multicolumn{1}{c}{HMDB}\\
       
	  \midrule
	   %XDC*~\cite{alwassel_2020_xdc} & IG65 & R(2+1)D+18 & 224    & 85.3 &56.0\\
	   %AVSF*~\cite{xiao2020audiovisual} & K400 & SF-50 & 224    & 77.4 & 42.2\\
	   MemDPC~\cite{han2020memory} & K400 & R-2D3D & 224    & 54.1 &30.5\\
	   CVRL~\cite{qian2021spatiotemporal} & K400 & R3D-50 & 224   & 89.8 &58.3\\
	   \hdashline[5pt/5pt]
	   Enhanced\cite{qian2021enhancing} & K400 & R3D+18&112   & 63.2 &33.4\\
	   CoCLR~\cite{Han20} & K400 & S3D& 128    & 74.5 &46.1\\
	   CoCLR+~\cite{Han20} & K400 & S3D& 128    & 77.8  &52.4\\
	   \textbf{GOCA} & K400 & S3D& 128 & 78.9  &50.5\\
	   \textbf{GOCA+} & K400 & S3D& 128   &\textbf{82.8}  &\textbf{58.7}\\
	   
	   %\midrule
	   % \midrule
	   %\textbf{GOCA} & UCF & R(2+1)D+18& 112   & 66.4  &38.0\\
	   %\textbf{GOCA+} & UCF & R(2+1)D+18 & 112 & \textbf{77.8}  &\textbf{49.5}\\
	    \midrule

	   CoCLR~\cite{Han20} & UCF & S3D& 128    & 70.2  &39.1\\
	   
	   CoCLR+~\cite{Han20} & UCF & S3D& 128    & 72.1  &40.2\\
	   ViCC~\cite{toering2021selfsupervised} & UCF & S3D& 128     & 72.2  &38.5\\
	   ViCC+~\cite{toering2021selfsupervised} & UCF & S3D& 128    & 78.0  &47.9\\
	   
	   \textbf{GOCA} & UCF & S3D& 128    & 69.2  &38.6\\
	   \textbf{GOCA+} & UCF & S3D& 128   & \textbf{80.1}  &\textbf{50.0}\\
	   \midrule
	\bottomrule
	\end{tabular}}}
	\caption{
  \emph{Linear Classification} experimental setup results on UCF101~\cite{ucf101} and HMDB\cite{hmdb}. \label{tbl:lc}
}
		
	
\end{table}


==> tbls/lc_ft.tex <==

\begin{table}[t]
    % \vspace{-6mm}
    \addtolength{\tabcolsep}{-1.5pt}    
	% %\setlength\tabcolsep{2 pt}
	\centering{
		\resizebox{.39\textwidth}{!}{
	\begin{tabular}{
			>{\raggedright\arraybackslash}p{2cm}
			>{\columncolor{Res2}}>{\centering\arraybackslash}p{0.7cm}
			>{\columncolor{Res2}}>{\centering\arraybackslash}p{1.7cm}
			>{\columncolor{Res2}}>{\centering\arraybackslash}p{0.5cm}
			>{\columncolor{Res1}}>{\centering\arraybackslash}p{0.7cm}
			>{\columncolor{Res3}}>{\centering\arraybackslash}p{1.1cm}}
	    
	    \multicolumn{6}{c}{\textbf{Linear Classification}} \\
	    
	    \midrule
		\multicolumn{1}{c}{Method}
		&\multicolumn{1}{c}{DS} 
		&\multicolumn{1}{c}{Backbone} 
		&\multicolumn{1}{c}{Res} 
		&\multicolumn{1}{c}{UCF}
		&\multicolumn{1}{c}{HMDB}\\
       
	  \midrule
	   %XDC*~\cite{alwassel_2020_xdc} & IG65 & R(2+1)D+18 & 224    & 85.3 &56.0\\
	   %AVSF*~\cite{xiao2020audiovisual} & K400 & SF-50 & 224    & 77.4 & 42.2\\
	   MemDPC~\cite{han2020memory} & K400 & R-2D3D & 224    & 54.1 &30.5\\
	   CVRL~\cite{qian2021spatiotemporal} & K400 & R3D-50 & 224   & 89.8 &58.3\\
	   \hdashline[5pt/5pt]
	   Enhanced\cite{qian2021enhancing} & K400 & R3D+18&112   & 63.2 &33.4\\
	   CoCLR~\cite{Han20} & K400 & S3D& 128    & 74.5 &46.1\\
	   CoCLR+~\cite{Han20} & K400 & S3D& 128    & 77.8  &52.4\\
	   \textbf{GOCA} & K400 & S3D& 128 & 78.9  &50.5\\
	   \textbf{GOCA+} & K400 & S3D& 128   &\textbf{82.8}  &\textbf{58.7}\\
	   
	   %\midrule
	   % \midrule
	   %\textbf{GOCA} & UCF & R(2+1)D+18& 112   & 66.4  &38.0\\
	   %\textbf{GOCA+} & UCF & R(2+1)D+18 & 112 & \textbf{77.8}  &\textbf{49.5}\\
	    \midrule
        \midrule
	   CoCLR~\cite{Han20} & UCF & S3D& 128    & 70.2  &39.1\\
	   
	   CoCLR+~\cite{Han20} & UCF & S3D& 128    & 72.1  &40.2\\
	   ViCC~\cite{toering2021selfsupervised} & UCF & S3D& 128     & 72.2  &38.5\\
	   ViCC+~\cite{toering2021selfsupervised} & UCF & S3D& 128    & 78.0  &47.9\\
	   
	   \textbf{GOCA} & UCF & S3D& 128    & 69.2  &38.6\\
	   \textbf{GOCA+} & UCF & S3D& 128   & \textbf{80.1}  &\textbf{50.0}\\
	   \midrule
	   %\\
	   %\vspace{-5mm}
	   \multicolumn{6}{c}{\textbf{Fine Tuning}} \\
	   \midrule
	   %XDC*~\cite{alwassel_2020_xdc} & K400 & R(2+1)D+18 & 224    & 84.2 &47.1\\
	   %AVSF*~\cite{xiao2020audiovisual} & K400 & SF-50 & 224    & 87.0 & 54.6\\
	   CVRL~\cite{qian2021spatiotemporal} & K400 & R3D-50 & 224   & 92.9 & 67.9\\
	   %MoCo~\cite{feichtenhofer2021large} & K400 &R-50 & 224    & 93.3 & - \\
	   $\rho$ BYOL~\cite{feichtenhofer2021large} & K400 &R-50 & 224     & 95.5 & 73.6 \\
	   %TaCo~\cite{bai2020can} & K400 & R50 & 224    & 85.1 & 51.6\\
	  \hdashline[5pt/5pt]
	   ASCNet\cite{qian2021enhancing} & K400 & R3D-18 & 112    & 80.5 &  52.3\\
	   Enhanced\cite{qian2021enhancing} & K400 & R3D-18 & 112    & 79.1 &  47.6\\
	   CoCLR~\cite{Han20} & K400 & S3D & 128    & 87.9 & 54.6\\
	   CoCLR+~\cite{Han20} & K400& S3D & 128  & 90.6 &
	   62.9\\
	   
	   
	   \textbf{GOCA} & K400 & S3D & 128    & 89.3 & 63.2\\
	   \textbf{GOCA+} & K400 & S3D & 128    & \textbf{91.1} &
	   \textbf{65.8}\\
	   \midrule
	   \midrule
	   %VCOP~\cite{xu2019self} & UCF & R(2+1)D+18 & 112    &  72.4 &  30.9\\
	    
	   Var. PSP~\cite{cho2021self} & UCF & R3D+18 & 112    &  74.8 &  36.8\\
	      
	   PacePred~\cite{wang2020self} & UCF & R(2+1)D+18 & 112     &  75.9 & 35.9\\
	   VCP~\cite{luo2020video} & UCF & R(2+1)D+18 & 112    &  66.3 & 32.2\\
	   PRP~\cite{Yao_2020_CVPR} & UCF1 & R(2+1)D+18 & 112    & 72.1 & 35.0\\
	   RTT~\cite{jenni2020video} & UCF & R(2+1)D+18 & 112    & 81.6 & 46.4\\
	   Enhanced~\cite{qian2021enhancing} & UCF & R3D+18 & 112    & 76.2 &  41.1\\
	   
	   \textbf{GOCA} & UCF & R(2+1)D+18 & 112     &  82.1 &   54.7\\
	   \textbf{GOCA+} & UCF & R(2+1)D+18 & 112    & \textbf{88.7} &  \textbf{60.1} \\
	 
	  \midrule
	 
	 
	   CoCLR~\cite{Han20} & UCF & S3D & 128   & 81.4 & 52.1\\
	   CoCLR+~\cite{Han20} & UCF & S3D & 128    & 87.3 &  58.7\\
	   ViCC~\cite{toering2021selfsupervised} & UCF & S3D & 128    &  84.3 &   47.9\\
	   ViCC+~\cite{toering2021selfsupervised} & UCF & S3D & 128    & \textbf{90.5} &   62.2\\
	   
	   \textbf{GOCA} & UCF & S3D & 128     &  83.4 &   53.5\\
	   \textbf{GOCA+} & UCF & S3D & 128  & 90.2 &  \textbf{64.8}\\
	\bottomrule
	\end{tabular}}}
	\setlength{\belowcaptionskip}{\RemoveBelowCaption}
	\caption{Top-1 classification accuracy results. 
}
		\label{tbl:lc_ft}
\end{table}

